Learning Collaborative Agents with Rule Guidance for Knowledge Graph Reasoning

Walk-based models have shown their advantages in knowledge graph (KG) reasoning by achieving decent performance while providing interpretable decisions. However, the sparse reward signals offered by the KG during traversal are often insufficient to guide a sophisticated walk-based reinforcement learning (RL) model. An alternate approach is to use traditional symbolic methods (e.g., rule induction), which achieve good performance but can be hard to generalize due to the limitation of symbolic representation. In this paper, we propose RuleGuider, which leverages high-quality rules generated by symbolic-based methods to provide reward supervision for walk-based agents. Experiments on benchmark datasets show that RuleGuider improves the performance of walk-based models without losing interpretability.

==> src/5-Related_work.tex <==
\section{Related Work}
%Prior arts on KG reasoning can be categorized into three lines.

\start{Symbolic-based methods~} reveal symbolic patterns of relation paths in the form of first-order logic rules.
Early works include FOIL and its follow-up works\cite{quinlan1990learning,landwehr2007integrating,landwehr2010fast}.
%Despite of their success, they suffer from high complexity and can hardly scale to large graphs.
Later, AMIE and AMIE+\cite{galarraga2013amie,galarraga2015fast} is developed for efficient mining without counterexamples.
Recently, AnyBURL \cite{Meilicke2019AnytimeBR,meilicke2020reinforced} shows comparable performance to the state-of-the-art methods with significant advantages in efficiency.

\start{Embedding-based methods~} learn distributed representations of entities and relations, and evaluate a target triple with a matching function using corresponding representations.
%for a target triple with distributed representation, and thus can capture rich semantic information of entities and relations
\cite{Bordes2013TranslatingEF,Socher2013ReasoningWN,Yang2014EmbeddingEA,Trouillon2016ComplexEF,Dettmers2017Convolutional2K,Zhang2018DiscriminativePK,Sun2019RotatEKG}.
They achieved superior performance but still lack of interpretability.
%However, they are one-hop prediction models that ignore complex patterns for complete reasoning paths. They are also short of interpretability for their embeddings and matching functions.

%\start{Reasoning-based methods~}
\start{Walk-based methods~}
capture advantages of both symbolic and embedding representations to generate reasoning paths~\cite{xiong2017deeppath,das2017go,shen2018reinforcewalk,chen2018variational}. %a comprehensive reasoning path.% from the query entity to the target entity.
%Following the pioneers~\cite{xiong2017deeppath,das2017go}, works on this line learn a RL model to generate the multi-hop decision sequence \cite{shen2018reinforcewalk,chen2018variational}.
%Such algorithms can suffer from inaccurate reward given by the incomplete input graph.
%To alleviate this problem, 
Recently, Multi-Hop model \cite{lin-etal-2018-multi-hop} is proposed to leverage pretrained embeddings to measure rewards in a RL model.
%models to compensate for false-negative rewards given by the incomplete graph.

%In this work, we explore to incorporate advantages of all three kinds of models, to develop a novel pattern-guided multi-hop reasoning model.

